ASTRA: Accurate and Scalable ANNS-based Training of Extreme Classifiers

`Extreme Classification'' (or XC) is the task of annotating data points (queries) with relevant labels (documents), from an extremely large set of $L$ possible labels, arising in search and recommendations. The most successful deep learning paradigm that has emerged over the last decade or so for XC is to embed the queries (and labels) using a deep encoder (e.g. DistilBERT), and use linear classifiers on top of the query embeddings. This architecture is of appeal because it enables millisecond-time inference using approximate nearest neighbor search (ANNS). The key question is how do we design training algorithms that are accurate as well as scale to $O(100M)$ labels on a limited number of GPUs. State-of-the-art XC techniques that demonstrate high accuracies (e.g., DEXML, Ren\'ee, DEXA) on standard datasets have per-epoch training time that scales as $O(L)$ or employ expensive negative sampling strategies, which are prohibitive in XC scenarios. In this work, we develop an accurate and scalable XC algorithm ASTRA with two key observations: (a) building ANNS index on the classifier vectors and retrieving hard negatives using the classifiers aligns the negative sampling strategy to the loss function optimized; (b) keeping the ANNS indices current as the classifiers change through the epochs is prohibitively expensive while using stale negatives (refreshed periodically) results in poor accuracy; to remedy this, we propose a negative sampling strategy that uses a mixture of importance sampling and uniform sampling. By extensive evaluation on standard XC as well as proprietary datasets with 120M labels, we demonstrate that ASTRA achieves SOTA precision, while reducing training time by 4x-15x relative to the second best.

==> main/figures/1k_dataset_1.tex <==
\begin{figure}
  \centering
  \subfloat[a][LF-AmazonTitles-1K]{\includegraphics[width=0.7\columnwidth]{main/figures/1k_datasets_1.png} \label{fig:a}} \\
  \subfloat[b][XXX]{\includegraphics[width=0.7\columnwidth]{main/figures/1k_datasets_1.png} \label{fig:b}}
  \caption[width=1\columnwidth]{Training time versus P@1 for \renee{}, \lexus{} with different negative sampling strategies across 2 datasets. \textit{Stale hard} uses stale query embeddings and classifier weights to generate hard negatives. \textit{Up-to-date hard} builds an ANNS index on classifier weights  and compute query embeddings every iteration to generate hard negatives. \lexus{} uses random negatives in addition to stale hard negatives. The markers on the lines indicate epoch completion (in multiples of 5). Takeaways: Up-to-date hard negatives gives the SOTA accuracy but is very inefficient. Adding random negatives to stale hard negatives makes it orders of magnitude efficient without any loss of accuracy.} 
\label{fig:motivation}
\end{figure}



==> main/figures/rq_1.tex <==

\begin{figure*}
\begin{tabular}{@{}c@{}c@{\hspace{-2mm}}c@{}}
\scalebox{0.95}{
\includegraphics[width=0.7\columnwidth]{main/figures/lfat131k.png}
}
&
\scalebox{0.95}{
\includegraphics[width=0.7\columnwidth]{main/figures/wiki.png}
}
&
\scalebox{0.95}{
\includegraphics[width=0.7\columnwidth]{main/figures/epm20m.png}
\label{fig:epm20m}
}
\\
(a) LF-AmazonTitles-131K & (b) LF-Wikipedia-500K & (c) SS-20M
\end{tabular}
\vspace*{-5pt}
\caption{Training time versus P@1 for \renee{} and \lexus{} across 3 datasets. The markers on the lines indicate epoch completion (in multiples of 5). Takeaways: \red{??}.}
\label{fig:intro}
\end{figure*}



==> main/tables/cpu_ram.tex <==


\begin{table*}[]
\caption{This table contains the size of memmap files used to save retrieved hard negatives from ANNS index. This is equivalent to the additional RAM used during training of \lexus{} compared to \renee } 
 \label{tab:cpu_ram}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c}
\hline
\textbf{Dataset} & LF-AmazonTitles-131K & LF-Amazon-131K & Amazon-670K & LF-AmazonTitles-1.3M & Amazon-3M \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Additional \\ CPU RAM(GB)\end{tabular}} & 0.76 & 0.38 & 2.5 & 3.2 & 10.6 \\ \hline
\end{tabular}
}
\end{table*}


==> main/tables/gpu_mem.tex <==

\begin{table*}[]
\caption{This table compares the GPU memory usage of \lexus{} and \renee{} for classifier forward pass. Memory usage for the rest of the steps is same for both \lexus{} and \renee{}. Negative sampling in \lexus{} leads to upto 351x reduction in GPU memory usage.} 
 \label{tab:gpu_mem}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c}
\hline
\textbf{Dataset} & LF-AmazonTitles-131K & LF-Amazon-131K & Amazon-670K & LF-AmazonTitles-1.3M & Amazon-3M \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}Additional \\ CPU RAM(GB)\end{tabular}} & 0.76 & 0.38 & 2.5 & 3.2 & 10.6 \\ \hline
\end{tabular}
}
\end{table*}

